The Newtonian limit for perfect fluids

We prove that there exists a class of non-stationary solutions to the Einstein-Euler equations which have a Newtonian limit. The proof of this result is based on a symmetric hyperbolic formulation of the Einstein-Euler equations which contains a singular parameter $\ep = v_T/c$ where $v_T$ is a characteristic velocity scale associated with the fluid and $c$ is the speed of light. The symmetric hyperbolic formulation allows us to derive $\ep$ independent energy estimates on weighted Sobolev spaces. These estimates are the main tool used to analyze the behavior of solutions in the limit $\ep \searrow 0$.

==> EE.tex <==
\sect{EE}{Einstein-Euler equations}

The Einstein-Euler equations or, in other words, the Einstein equations
coupled to a simple perfect fluid are given by the following system of equations
\lgath{EEeqn}{
G^{ij} = \frac{8\pi G}{c^4} T^{ij} \label{EEeqn.1} \\
\nabla_{i} T^{ij} = 0 \label{EEeqn.2} } where the stress-energy
tensor for the fluid is given by \lgath{EEdefs}{ T^{ij} = (\rho +
c^{-2} p)v^i v^j + p g^{ij} \,  } with $\rho$ the fluid density,
$p$ the fluid pressure, and $v$ the fluid four-velocity normalized
by $v^iv_i = -c^2$. Here $c$ is the speed of light and $G$ is the
Newtonian gravitational constant. We will only consider isentropic
flow where the pressure is related to the density by an equation
of state of the form $p = f(\rho)$

In formulating a symmetric hyperbolic system for the fluid
variables $\{\rho,v\}$, we need to deal with the well known
problem that the system becomes singular when $\rho + c^{-2} p =
0$. This is a particular problem for fluid balls having compact
support. To get around this problem, we will follow Rendall
\cite{Ren92} and use a technique of Makino \cite{Mak} to
regularize the fluid equations so a class of gravitating fluid
ball solutions can be constructed. Thus as in \cite{Ren92}, we
assume an equation of state of the form \leqn{eos}{ p =
K\rho^{(n+1)/n} } where $K \in \Rbb_{>0}$, $n\in \Nbb$, and we
introduce a new ``density'' variable $\alpha$ via the formula
\leqn{dendef}{ \rho = \frac{1}{\bigl(4Kn(n+1)\bigr)^n}\alpha^{2n}
\, . } As discussed by Rendall, the type of fluid solutions
obtained by this method have freely falling boundaries and hence
do not not include static stars of finite radius  and so this
method is far from ideal. However, in trying to understand the
Newtonian limit and post-Newtonian approximations these solutions
are almost certainly general enough to obtain a comprehensive
understanding of the mathematical issues involved in the Newtonian
limit and post-Newtonian approximations. We would also like to
remark that the results contained in this article are largely
independent of the specific structure of the fluid equations. We
therefore expect that the analysis in this paper can be carried
over without much difficulty to other matter models whose
equations can be formulated as a symmetric hyperbolic system and
have a finite propagation speed for the matter density in the
limit $\ep\searrow 0$.


For the remainder of this article, we will assume that
spacetime $M$ is a manifold of the
form $M=S\times I\subset \Rbb^4$ where $S\cong \Rbb^3$ and $I\subset \Rbb$
is an open interval
containing $0$. We will always let capital Roman indicies, i.e. I,J,K etc.,
run from $1$ to $3$ and small Roman indicies, i,j,k etc., run from
$1$ to $4$. All equations will be formulated with respect
to a global set of Cartesian coordinates $(x^i,i=1,..4)$
on $M$ where $(x^I)$ are spatial coordinates that cover $S$
and $x^4$ is a ``time coordinate''
that covers the interval $I$.

